On a trace formula for functions of noncommuting operators

The main result of the paper is that the Lifshits--Krein trace formula cannot be generalized to the case of functions of noncommuting self-adjoint operators. To prove this, we show that for pairs $(A_1,B_1)$ and $(A_2,B_2)$ of bounded self-adjoint operators with trace class differences $A_2-A_1$ and $B_2-B_1$, it is impossible to estimate the modulus of the trace of the difference $f(A_2,B_2)-f(A_1,B_1)$ in terms of the norm of $f$ in the Lipschitz class.

==> classstartscr.tex <==
\setlength{\topmargin}{.1in}
\setlength{\textheight}{8in}
\setlength{\textwidth}{5.8in}
\setlength{\evensidemargin}{.4in}
\setlength{\oddsidemargin}{.4in}
%\newmathalphabet*{\bit}{cmm}{b}{it}

\newcommand{\lb}{\linebreak}
\newcommand{\noi}{\noindent}
\newcommand{\nl}{\newline}

\let\pl = \l
\let\PL = \L

%\let\pol=\l
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\vk}{\varkappa}
\newcommand{\z}{\zeta}
\newcommand{\ta}{\theta}
\newcommand{\vt}{\vartheta}
\renewcommand{\l}{\lambda}
\newcommand{\ro}{\rho}
\newcommand{\s}{\sigma}
\renewcommand{\t}{\tau}
\newcommand{\var}{\varphi}
\newcommand{\f}{\varphi}
\renewcommand{\o}{\omega}
\newcommand{\w}{\omega}
\newcommand{\G}{\Gamma}
\newcommand{\D}{\Delta}
\renewcommand{\L}{\Lambda}
\newcommand{\Sig}{\Sigma}
\renewcommand{\O}{\Omega}
\newcommand{\U}{\Upsilon}

\newcommand{\n}{\nabla}

\newcommand{\A}{{\mathscr A}}
\newcommand{\B}{{\mathscr B}}
\newcommand{\cc}{{\mathscr C}}
\newcommand{\E}{{\mathscr E}}
\newcommand{\cd}{{\mathscr D}}
\newcommand{\F}{{\mathscr F}}
\newcommand{\Q}{{\mathscr Q}}
\newcommand{\h}{{\mathscr H}}
\newcommand{\I}{{\mathscr I}}
\newcommand{\PQ}{{\mathscr J}}
\newcommand{\K}{{\mathscr K}}
\newcommand{\cL}{{\mathscr L}}
\newcommand{\M}{{\mathscr M}}
\newcommand{\N}{{\mathscr N}}
\newcommand{\p}{{\mathscr P}}
\newcommand{\cp}{{\mathscr P}}
\newcommand{\cR}{{\mathscr R}}
\newcommand{\cS}{{\mathscr S}}
\newcommand{\X}{{\mathscr X}}
\newcommand{\Y}{{\mathscr Y}}
\newcommand{\cU}{{\mathscr U}}
\newcommand{\V}{{\mathscr V}}
\newcommand{\W}{{\mathscr W}}

\newcommand{\sh}{{\bf S}}
\newcommand{\1}{{\bf 1}}


\newcommand{\C}{{\Bbb C}}
\newcommand{\T}{{\Bbb T}}
\newcommand{\pp}{{\Bbb P}}
\newcommand{\dd}{{\Bbb D}}
\newcommand{\R}{{\Bbb R}}
\newcommand{\Z}{{\Bbb Z}}
\newcommand{\mm}{{\Bbb M}}
\newcommand{\0}{{\boldsymbol{0}}}
\newcommand{\bO}{\{ {\mathbbb O} \}}

\newcommand{\bs}{\boldsymbol}
\newcommand{\PP}{{\boldsymbol{\cal P}}}
\newcommand{\PPt}{{\boldsymbol{\tilde{\cal J}}}}
\newcommand{\BJ}{{\boldsymbol J}}
%\newcommand{\BJi}{{\bbi J}}
\newcommand{\BS}{{\boldsymbol{\cal S}}}
\newcommand{\DD}{{\boldsymbol{\cal D}}}
\newcommand{\GG}{{\boldsymbol{\varGamma}}}
\newcommand{\m}{{\boldsymbol m}}
\newcommand{\bS}{{\boldsymbol S}}


\newcommand{\bb}[1]{\mbox{{\boldmath$#1$\unboldmath}}}
\newcommand{\bbo}[1]{\mbox{\rm{\bf #1}}}
\newcommand{\cs}{\mbox{\rm const}\cdot}
\newcommand{\rf}[1]{(\ref{#1})}
\newcommand{\cl}[1]{{\cal #1}}
\newcommand{\hh}[1]{\breve{#1}}
\newcommand{\col}{\mbox{\rm col}}
\newcommand{\tx}[1]{\mbox{\rm{#1}}}


%\newcommand{\operatorname}[1]{{\rm#1\,}}
\newcommand{\df}{\stackrel{\mathrm{def}}{=}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\Ker}{\operatorname{Ker}}
\newcommand{\re}{\operatorname{Re}}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\clos}{\operatorname{clos}}
\newcommand{\convh}{\operatorname{convh}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\const}{\operatorname{const}}
\newcommand{\tr}{\operatorname{trace}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\bay}{\begin{eqnarray}}
\newcommand{\ba}{\begin{align*}}
\newcommand{\ea}{\end{align*}}
\newcommand{\ey}{\end{eqnarray}}
\newcommand{\bey}{\begin{eqnarray*}}
\newcommand{\eey}{\end{eqnarray*}}
\newcommand{\os}{\mbox{\small $\bigcirc$}\hspace*{-.23cm}\mbox{\small s}\;}
\newcommand{\tos}{\mbox{\tiny $\bigcirc$}\hspace*{-.2cm}\mbox{\tiny s}}
\newcommand{\ra}{\rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\eq}{\Leftrightarrow}
\newcommand{\imp}{\Rightarrow}
\newcommand{\be}{\infty}
\newcommand{\bib}{thebibliography}
\newcommand{\bl}{\blacksquare}
\newcommand{\ess}{\operatorname{ess}}
\newcommand{\ind}{\operatorname{ind}}
\newcommand{\wind}{\operatorname{wind}}
\newcommand{\Range}{\operatorname{Range}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Pf}{{\bf Proof. }}
%\newcommand{\qed}{\mbox{$\Box$}}
\newcommand{\im}{\operatorname{Im}}
\renewcommand{\re}{\operatorname{Re}}
\newcommand{\ov}{\overline}






\def\mathR{\mbox{$\bf \rm I\makebox [1.2ex] [r] {R}$}}


\newtheorem{thm}{\hspace{\parindent}Theorem}[section]
\newtheorem{prop}[thm]{\hspace{\parindent}Proposition}
\newtheorem{cor}[thm]{\hspace{\parindent}Corollary}
\newtheorem{lem}[thm]{\hspace{\parindent}Lemma}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{exa}[thm]{Example}
\newtheorem{defn}[thm]{Definition}



\newcommand{\Qed}{\mbox{$\Box$} \medskip}
\newcommand{\pams}{Proc. Amer. Math. Soc.}
\newcommand{\tams}{Trans. Amer. Math. Soc.}
\newcommand{\dmj}{Duke Math. J.}
\newcommand{\aim}{Adv. in Math.}
\newcommand{\cjm}{Canad. J. Math.}
\newcommand{\pjm}{Pacific J. Math.}
\newcommand{\plms}{Proc. London Math. Soc.}
\newcommand{\jram}{J. Reine Angew. Math.}
\newcommand{\sv}{Springer-Verlag Lecture Notes in Math.}
\newcommand{\caup}{Cambridge University Press}
\newcommand{\oup}{Oxford University Press} 
\newcommand{\pr}{preprint}
\newcommand{\ip}{in preparation}


